Cross-document Event Coreference Search: Task, Dataset and Modeling

The task of Cross-document Coreference Resolution has been traditionally formulated as requiring to identify all coreference links across a given set of documents. We propose an appealing, and often more applicable, complementary set up for the task - Cross-document Coreference Search, focusing in this paper on event coreference. Concretely, given a mention in context of an event of interest, considered as a query, the task is to find all coreferring mentions for the query event in a large document collection. To support research on this task, we create a corresponding dataset, which is derived from Wikipedia while leveraging annotations in the available Wikipedia Event Coreference dataset (WEC-Eng). Observing that the coreference search setup is largely analogous to the setting of Open Domain Question Answering, we adapt the prominent Deep Passage Retrieval (DPR) model to our setting, as an appealing baseline. Finally, we present a novel model that integrates a powerful coreference scoring scheme into the DPR architecture, yielding improved performance.

==> sections/bkp/data_create_bkp.tex <==
\section{The \weces{} Dataset}
\label{sec:data_create}
Following our Cross-Document Coreference Event-Search task formulation, we created a new dataset (\weces{}) tailored for the task. We now describe the process we used to create \weces{}. We start by describing \weces{} format (§\ref{sec:dataset-format}), following by a description of \weces{} creation methodology (§\ref{sec:creat-method}).


\subsection{High-Level \weces{} Dataset Format}
\label{sec:dataset-format}
Our \weces{} dataset consists of two separate collections: A collection of coreferring passages containing manually annotated event mentions taken from \wecEng{}, and a collection of destructor passages without any annotation (containing only context). A single passage instance in the manually annotated collection, can take the role of either a query, a positive passage for a query belonging in the same coreferring cluster or a negative passage to any query not belonging within its coreference cluster. The set of destructor passages can only be considered as non-relevant passages in the passage collection (see Table~\ref{tab:weces-stats} for the full dataset statistics). 


\input{tables/clusters}

\subsection{\weces{} Creation Methodology}
\label{sec:creat-method}
We facilitated a process where \weces{} dataset is created using the validated portion of \wecEng{} \cite{eirew-etal-2021-wec} corpus (§\ref{sec:cdec-datasets} and Table~\ref{tab:wecEng-stats}). To that end, we merged \wecEng{} test and development sets clusters into a single collection of 522 none-singleton clusters (we excluded singleton clusters, as those can only contribute negative examples).\footnote{Merging \wecEng{} development and test set is legitimate since mention cannot corefere between clusters, thus no data leakage between development and test set possible.}

Then, we sampled 49 clusters for our \weces{} development set and split the remaining 473 clusters between the test and train sets. 
(see ``Validated Clusters'' in Table~\ref{tab:weces-stats}). Each coreference cluster consists of a set of passages, where each instance contains the event mention span surrounded by its context as well as its coreference cluster identification. For the transformation from coreference clusters to queries and passages collections, we iterate over all cluster mentions in the following way; We select a single passage to donate a query containing the mention span and use the rest of the cluster passages as positive examples. 

Up to this point, we used \wecEng{} development and test sets to facilitate a collection of queries and positive passages. We now describe the process used to create a realistic large passage collection. To generate negative passages (i.e., destructing passages), we used three resources: (1) for every cluster now belonging to \weces{} development and test sets, we used all other cluster mentions (from the same set) as negative examples. (2) We divided \wecEng{} train mentions between \weces{} development, test, and train splits (see ``Passages All'' in Table~\ref{tab:weces-stats}). (3) After the above steps, our passage collection for retrieval was still rather small (roughly 14,500 passages per query) when compared to common open-domain question answering dataset \cite{berant-etal-2013-semantic, baudi-etat-2015, joshi-etal-2017-triviaqa, kwiatkowski-etal-2019-natural, rajpurkar-etal-2016-squad}. 

Therefore, we further expand the passage collection from Wikipedia. According to Wikipedia Manual of Style, authors should add a link to a Wikipedia page at the first appearance of an event in the article.\footnote{\href{https://en.wikipedia.org/wiki/Wikipedia:Manual\_of\_Style/Linking\#Duplicate\_and\_repeat\_links}{Wikipedia Manual-of-Style (Linking)}} Following, we extracted the first paragraph of every Wikipedia article, and then filtered any paragraph containing a link referring to one of the event mention available in \wecEng{} development or test sets clusters. Using this method, we where able to collect in total 2,729,296 additional negative passages examples (see ``Added Negative Passages'' in Table~\ref{tab:weces-stats}).

\paragraph{Cluster Types}
The process described in §\ref{sec:creat-method} results with queries and positive passage examples, belonging to the same cluster. We distinguish between two types of clusters: \textit{Type-1} - clusters containing only passages with event mentions spans that include the event time or location (e.g., ``2006 Dahab bombings'', ``2013's BET Awards'') and \textit{Type-2} - clusters that are comprised of both passages as in Type-1, as well as passages containing mention span without any event identifying arguments (e.g., ``the deadliest earthquake on record'', ``BET Awards'', ``plane crash''). Naturally, Type-2 clusters will create queries/passage examples with a higher degree of difficulty. This due to \wecEng{} multitude of event mention having similar lexical representation which do not corefere \cite{eirew-etal-2021-wec}, requiring a model to identify the event using the arguments in the surrounding context.

To measure the distribution of cluster types within \weces{}, we randomly sampled 20 clusters and found 90\% are of type-2. Table~\ref{tab:clusters} present example of queries extracted randomly from the first five type-2 clusters we extracted.

\paragraph{Potential Language Adaptation}
\weces{} dataset is built on top of the English version of WEC (i.e., \wecEng{}). Consequently, since WEC is adoptable to other languages \cite{eirew-etal-2021-wec}, and the process described above (§\ref{sec:creat-method}) is simple and does not require any specific language adaptations, \weces{} dataset can be adopted to other languages as well (assuming the availability of WEC dataset in other languages). 


==> sections/bkp/dump.tex <==
% ### CorefQA Dump ###

\subsubsection{Integrated DPR and Coreference Scoring} 
\label{sec:coref-integrated}
Above DPR baseline model yield appealing performance (as we show next in §\ref{sec:e2e-results}). However, we hypothesize that DPR passage selection (equation \ref{eq:select}) is sub-optimal for coreference resolution. To test our assumption, we replaced the passage selection component in DPR with components inspired by the within document end-to-end coreference resolution model \cite{lee-etal-2017-end}.

We adjust the query-based span prediction model \cite{wu-etal-2020-corefqa} from the within-document (WD) coreference resolution task, to our task and dataset. Specifically, similar to previous works \aeinline{add citation}, we train two separate models, a \emph{mention proposal} model and a \emph{span prediction} model. The mention proposal model, learn a mention score $s_m(i)$ for each mention $i$ within a query/passage, by taking the representation of the mention start/end tokens separately and the concatenation of the start and end tokens. We used RoBERTa (base, cased) for query and passage representation.

The span prediction model, uses cross attention between the query and the passage to learn an antecedent score $s_a(j|i)$, where $i$ represent the query and $j$ represent the passage. The learning is done once over the concatenation of the passage mention start and end tokens. Then alternating the cross attention such that the passage takes the query role and vise versa, and similarly compute the antecedent score $s_a(i|j)$. Overall, the antecedent final score $s_a(i,j)$ is calculated as the average of the sum of both $s_a(j|i)$ and $s_a(i|j)$ scores. Finally, the pairwise score for query/passage pair is calculated as: 
\begin{equation}
s(i,j)=\lambda[s_m(i) + s_m(j)] + (1 - \lambda)s_a(i,j)
\end{equation}

We aim to optimize the marginal log-likelihood of all correct antecedents implied by the gold clustering.

%\begin{equation}
%\begin{split}
%S_m(i)=[FFNN([x_{FIRST(i)}]) + \\ FFNN([x_{LAST(i)}]) \\ + FFNN([x_{FIRST(i)}, %x_{LAST(i)}])]/3
%\end{split}
%\end{equation}

\paragraph{Query Representation} Similarly to the retriever query representation, we applied in the boundary tokens (<QSPAN-START> and <QSPAN-END>) to mark the query mention span within the query context, this presented a significant improvement both in span prediction and re-ranking in our experiments.

\paragraph{Training} At training, for each query $q$, we sample one positive passage (sampled from $q$ cluster) and m(=24) negative passages, selected from the top passages returned (by our best retrieval system) for $q$, in case no positive in the top results the query is discarded. We repeat this query selection for each query in the cluster and for each cluster in our dataset. The training objective is to optimize the cross entropy loss over the passages gold spans.

\paragraph{Inference} At inference, we apply the end-to-end system, thus, for each query, first the retriever model extract the top-k passages from the passage collection, then the reader model will re-rank and attempt to extract the coreference mention span from the returned passages. 

%Next, given a query top-k retrieved results at inference time, the reader component will be comprised of a single BERT model for representing each passage. The reader model will serve two objectives: 1) a re-ranker, through cross attention between the question and the passage (instead of the similarity function, now made possible due to the much smaller number of passages candidates); and 2) an answer selector, made possible by learning three additional vectors, for optimizing the start, end and selection part probabilities of each retrieved passage. The training, similar to the retriever, is done on a sample of one positive and N negative examples for each query. The objective is to maximize the marginal log-likelihood of all the correct answer spans in the positive passage, combined with the log-likelihood of the positive passage being selected.


% #### From Data Creation #####
%Notably, gold mention span annotation within passages, should only be available to the model during training, as one of the task goals is detecting the mention span in the retrieved passage. However, at inference, only the query mention span should be available to the model. 
%\ac{I merged this sentence with the paragraph. Also, this should be attached to the discussion about mentions and not about passages.}

% \weces{} dataset statistics are covered in Table~\ref{tab:weces-stats} 

%Our goal in creating \weces{} Dataset, was to establish a dataset which present two main characteristics for our formulated event-coreference search task: 1) Present clean and validated data of queries and passages containing a coreferring mention between them. 2) Consist of a large collection of passages to establish a challenging retrieval task. 

% \subsection{Wikipedia Event Coreference Dataset}
% \label{sec:wec_eng}

% %\ac{I'd spend here a paragraph briefly describing the task the WEC induces before describing it.}
% \ac{If this appears at the BG, no need for it twice.}
% The \weces{} dataset is based on the Wikipedia Event Coreference dataset for the English language (\wecEng{}) \citep{eirew-etal-2021-wec}. \wecEng{} was created to support the development of cross-document event coreference algorithms. This dataset distinguish from previous CDEC dataset in two aspects: (1) it in not partitioned into separate topics, thus, events can corefer across the entire corpus. (2) mention annotations is not exhaustive, at each instance, only a single mention is annotated. Therefore, coreference resolution can only be performed over the gold mentions. 

% Our decision to adopt \wecEng{} to our task was motivated by those two aspects, which align with our task formulation. 

% \wecEng{} was gathered automatically by clustering together anchor texts of (internal) Wikipedia links pointing to the same Wikipedia concept. Accordingly, this dataset consists of a set of mentions, where each one includes the span corresponding to the link anchor text, the surrounding context (paragraph), and the cluster identification link.

% \wecEng{} is split into train, development and test sets (presented in Table~\ref{tab:wecstats}). The larger train set, contains 40,529 event mentions and 7,042 clusters, was derived using a fully automatic process and therefore contains some erroneous mentions, roughly estimated by the authors at 17\% of the mentions. On the other hand, the much smaller development set (containing 1,250 mentions and 233 clusters) and test set (contains 1,893 mentions and 322 clusters), have gone a manual validation process.



==> sections/task.tex <==
\section{Task Formulation}
We motivate introducing a novel coreference search task by the observation that applicable cross-document event coreference resolution (CDEC) might be centered around finding coreferring event mentions to a particular event. 
A typical use-case can be of a user reading text, encounters upon an event of interest (for example, the \textit{plane crash} event in Figure~\ref{fig:figure_arch}), and would like to further explore and learn about the event from a large document resource.

Currently, the CDEC task, as formed in corresponding datasets, is intended at creating models that exhaustively resolve all coreference links in a given dataset (§\ref{sec:cdec-datasets}). 
%\ac{I think that this should be positioned towards the datasets, and not the models. I mean datasets dictate the task and not the models.} 
%This approach suffers from a prominent scalability and feasibility limitation, as it requires a quadratic time and memory complexity, creating a computational bottleneck when dealing with large datasets. Furthermore, applying this settings on real-world expanding resources (such as news, Wikipedia, court and police reports, etc.), where new events are added daily, might require re-running these computationally demanding models repeatedly. 

% We argue that in our fast past and digitized world, a more appropriate solution is required. In some realistic scenarios, it is only required to search events which corefer with a single provided event. Good examples of such systems are information retriever \cite{Dietz2018TRECCA}, \emph{interactive} multi-document summarization \citep{leuski2003ineats, shapira2020evaluating, hirsch-etal-2021-ifacetsum}, multi-hop question answering \citep{dhingra-etal-2018-neural, wang-etal-2019-multi-hop} and search engines (e.g., Google, Bing, Yahoo and so on). \ac{this is not really a limitation since you can apply the coref models over a single mention as a query.\aeinline{Not sure I understand what you mean?}}

To support the use-cases described above, we formulated the \textit{Cross-Document Event Coreference Search} task following a similar approach to open-domain question answering (illustrated in Figure~\ref{fig:figure_arch}). Specifically, given a query containing an event mention, along with a passage collection, the goal is to return all the passages from the passage collection, containing event mention coreferring with the event mention in query, and extracting the mention span. 

Given this task definition, a suitable dataset should consist of a collection of passages and a sample of queries containing event mentions.

% provided with a large collection of passages, a single passage instance representing the query, which is provided along with annotation of an event mention span. The goal of CDeS system, is to return a ranked list of [\textit{passage identification}, \textit{mention span}] pairs per question such that each mention span string was believed to contain the mention coreferring with the event mention in the query.

% set of coreference clusters, where each cluster instance contains [\textit{context}, \textit{passage identification}, \textit{mention indexes in context}, \textit{coreference identification}], and optionally if needed a set of destructor passages containing only a context.

Notably, we distinguish between the visibility of mention spans within passages at training or at inference. Providing the span of the event as part of the query is necessary for both training and inference \ac{, in order to enable the search of particular events}, however passages within the search collection should not include any mention annotation at inference, but only as part of model training.

%Notably, we distinguish between the visibility of the gold spans at training or at inference. In a realistic scenario, while providing the span of the event as part of the query seems legitimate and even necessary, expecting the searched dataset to have annotated event mentions is less realistic. Thus, we expect the passages within the searched dataset to have no additional information attached to them at inference time, but to return only as part of model training.

Last, in order to evaluate a CDES system, given a query and candidate passages returned by a CDES system, we follow two simple rules: (1) Passage is considered as relevant, if and only if the passage contains an event mention coreferring with query event. (2) Extracted event mention from retrieved passage is considered as correct, if and only if the extracted mention span indexes equal the gold annotation indexes (we further discuss evaluation in §\ref{sec:eval}).

%the set of gold annotation, a model should be rewarded only for retrieving passages containing a gold mention coreferring with query mention (we further discuss evaluation in §\ref{sec:eval}). 

%\ac{There is not task formulation here at all! only motivation. Please add mathematical definition of the problem, and what is the goal. Please refer to the DPR paper for an example.}
%Lastly, similar to within-document and cross-document tasks, \textit{Cross-Document Coreference Event-Search} systems should also predict the span of the corefering mention within the retrieved passages.

%\begin{itemize}
    %\item Motivation - What we would like to achieve and why
    %\begin{itemize}
     %   \item A method for search efficiantly for events that corefere in a large passage collection
      %  \item we would like to be able to both extract the most relevant passages as well as highlight the mention span within them
    %\end{itemize}
    %\item Describe/formulate the task - What is the expected input and output
%    \item point to the measurements in the model/evaluation part
 %   \item point to the example in the intro
%\end{itemize}

% \aeinline{Need to add: 1) point to the measurements in the model/evaluation part}
% \aeinline{Need to add: 2) point to the example in the intro}


==> tables/ablation.tex <==
\begin{table}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{@{}lcccccc@{}}
        \toprule
        \makecell{Model} & \makecell{MRR@10} & \makecell{mAP@10} & \makecell{mAP@25} & \makecell{R@10} & \makecell{R@100} & \makecell{R@500} \\
        \midrule
        BM25 & 57.32 & 25.92 & 29.88 & 27.63 & 56.09 & 74.75 \\
        Retriever-B & 23.56 & 4.91 & 6.51 & 9.53 & 42.66 & 65.09 \\
        Retriever-S & 75.4 & 37.6 & 42.55 & 40.06 & 71.65 & 86.21 \\
        \midrule
        Final & \textbf{80.92} & \textbf{40.43} & \textbf{46.06} & \textbf{41.59} & \textbf{74.03} & \textbf{87.53} \\
        \bottomrule
    \end{tabular}}
    \caption{Ablation study on retriever results on \weces{} development set. \textbf{BM25}: show BM25 results, \textbf{Retriever-B}: show DPR retriever using BERT and without boundary tokens, \textbf{Retriever-S}: shows DPR retriever using SpanBERT and without boundary tokens, and \textbf{Final}: Our final DPR retriever.}
    \label{tab:ablation-ret}
\end{table}


\begin{table}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{@{}lccccccc@{}}
        \toprule
        \makecell{Model} & \makecell{MRR@10} & \makecell{mAP@10} & \makecell{mAP@25} & \makecell{R@10} & \makecell{R@50} & \makecell{EM} & \makecell{F1} \\
        \midrule
        \multicolumn{8}{c}{\textbf{Dev}} \\
        \midrule
        $\mbox{E2E-DPR}^-$ & 89.81 & 58.19 & 66.34 & 55.16 & \textbf{84.47} & 74.99 & 82.97 \\
        $\mbox{E2E-DPR}^+$ & 92.48 & 58.23 & 64.1 & 53.34 & 73.81 & 79.59 & \textbf{88.91} \\
        \midrule
        $\mbox{E2E-Integrated}^-$ & TBD & TBD & TBD & TBD & TBD & TBD & TBD \\
        $\mbox{E2E-Integrated}^+$ & \textbf{94.05} & \textbf{61.82} & \textbf{69.15} & \textbf{56.53} & 82.19 & \textbf{83.31} & 88.78 \\
        \bottomrule
    \end{tabular}}
    \caption{Ablation study on end-to-end results on \weces{} development set. \textbf{E2E-DPR}: present our end-to-end DPR baseline. \textbf{E2E-Integrated}: indicate our integrated model without mention span boundary tokens. The '$^-$' indicate the model was trained without mention span boundary tokens, and '$^+$' with.}
    \label{tab:ablation-e2e}
\end{table}

